Disassociation energies for the finite density N-body problem

This paper considers the energy required for collections of finite density bodies to undergo escape under internal gravitational interactions alone. As the level of the system energy is increased there are different combinations of components that can escape, until the total energy becomes positive, when the entire system can undergo mutual disruption. The results are also defined for bodies modeled as a continuum. These results provide rigorous constraints for the disruption of rubble pile asteroids when only considering gravitational interaction effects, with the energy provided by rotation of an initial collection of the system. These issues are considered for discrete particles in the N body problem and for size distributions of discrete particles in the continuum limit.

==> CMDA_bilbiography.tex <==
\begin{thebibliography}{10}

\bibitem{andrews1998theory}
George~E Andrews.
\newblock {\em The theory of partitions}.
\newblock Number~2. Cambridge university press, 1998.

\bibitem{bell_number}
Daniel Berend and Tamir Tassa.
\newblock Improved bounds on bell numbers and on moments of sums of random
  variables.
\newblock {\em Probability and Mathematical Statistics}, 30(2):185--205, 2010.

\bibitem{toshi_1950DA}
M.~Hirabayashi and D.J. Scheeres.
\newblock {Stress and Failure Analysis of Rapidly Rotating Asteroid (29075)
  1950 DA}.
\newblock {\em The Astrophysical Journal Letters}, 798(1):L8, 2015.

\bibitem{holsapple_original}
KA~Holsapple.
\newblock Equilibrium configurations of solid cohesionless bodies.
\newblock {\em Icarus}, 154(2):432--448, 2001.

\bibitem{michikami}
T.~Michikami, A.M. Nakamura, N.~Hirata, R.W. Gaskell, R.~Nakamura, T.~Honda,
  C.~Honda, K.~Hiraoka, J.~Saito, H.~Demura, et~al.
\newblock {Size-frequency statistics of boulders on global surface of asteroid
  25143 Itokawa}.
\newblock {\em Earth, Planets, and Space}, 60(1):13--20, 2008.

\bibitem{moeckel2017minimal}
Richard Moeckel.
\newblock Minimal energy configurations of gravitationally interacting rigid
  bodies.
\newblock {\em Celestial Mechanics and Dynamical Astronomy}, 128(1):3--18,
  2017.

\bibitem{moeckel2018counting}
Richard Moeckel.
\newblock Counting relative equilibrium configurations of the full two-body
  problem.
\newblock {\em Celestial Mechanics and Dynamical Astronomy}, 130(2):17, 2018.

\bibitem{Pravec_clusters}
P.~Pravec, P.~Fatka, D.~Vokrouhlický, D.J. Scheeres, P.~Kušnirák,
  K.~Hornoch, A.~Galád, J.~Vraštil, D.P. Pray, Yu.N. Krugly, N.M. Gaftonyuk,
  R.Ya. Inasaridze, V.R. Ayvazian, O.I. Kvaratskhelia, V.T. Zhuzhunadze,
  M.~Husárik, W.R. Cooney, J.~Gross, D.~Terrell, J.~Világi, L.~Kornoš, Š.
  Gajdoš, O.~Burkhonov, Sh.A. Ehgamberdiev, Z.~Donchev, G.~Borisov, T.~Bonev,
  V.V. Rumyantsev, and I.E. Molotov.
\newblock Asteroid clusters similar to asteroid pairs.
\newblock {\em Icarus}, 304:110 -- 126, 2018.
\newblock Asteroids and Space Debris.

\bibitem{pravec_fission}
P.~Pravec, D.~Vokrouhlick{\`y}, D.~Polishook, D.J. Scheeres, AW~Harris,
  A.~Gal{\'a}d, O.~Vaduvescu, F.~Pozo, A.~Barr, P.~Longa, et~al.
\newblock Formation of asteroid pairs by rotational fission.
\newblock {\em Nature}, 466(7310):1085--1088, 2010.

\bibitem{sanchez_MAPS}
P.~S{\'a}nchez and D.J. Scheeres.
\newblock The strength of regolith and rubble pile asteroids.
\newblock {\em Meteoritics \& Planetary Science}, 49(5):788--811, 2014.

\bibitem{scheeres_F2BP}
D.J. Scheeres.
\newblock Stability in the full two-body problem.
\newblock {\em Celestial Mechanics and Dynamical Astronomy}, 83(1):155--169,
  2002.

\bibitem{scheeres_icarus_fission}
D.J. Scheeres.
\newblock Rotational fission of contact binary asteroids.
\newblock {\em Icarus}, 189(2):370--385, 2007.

\bibitem{scheeres_minE}
D.J. Scheeres.
\newblock {Minimum Energy Configurations in the $N$-Body Problem and the
  Celestial Mechanics of Granular Systems}.
\newblock {\em Celestial Mechanics and Dynamical Astronomy}, 113(3):291--320,
  2012.

\bibitem{F4BP_chapter}
D.J. Scheeres.
\newblock {Relative equilibria in the full $N$-body problem with applications
  to the equal mass problem}.
\newblock In {\em Recent Advances in Celestial and Space Mechanics}, pages
  31--81. Springer, 2016.

\bibitem{F3BP_scheeres}
D.J. Scheeres.
\newblock Relative equilibria in the spherical, finite density three-body
  problem.
\newblock {\em {Journal of Nonlinear Science}}, 26(5):1445--1482, 2016.

\bibitem{tsuchiyama_science}
A.~Tsuchiyama, M.~Uesugi, T.~Matsushima, T.~Michikami, T.~Kadono, T.~Nakamura,
  K.~Uesugi, T.~Nakano, S.A. Sandford, R.~Noguchi, et~al.
\newblock {{Three-Dimensional Structure of Hayabusa Samples: Origin and
  Evolution of Itokawa Regolith}}.
\newblock {\em Science}, 333(6046):1125--1128, 2011.

\bibitem{YORP_AIV}
David Vokrouhlicky, William~F Bottke, Steven~R Chesley, Daniel~J Scheeres, and
  Thomas~S Statler.
\newblock The yarkovsky and yorp effects.
\newblock {\em Asteroids IV. Univ. Arizona Press, Tucson}, 2015.

\end{thebibliography}

